MultiCoder: Multi-Programming-Lingual Pre-Training for Low-Resource Code Completion

Code completion is a valuable topic in both academia and industry. Recently, large-scale mono-programming-lingual (MonoPL) pre-training models have been proposed to boost the performance of code completion. However, the code completion on low-resource programming languages (PL) is difficult for the data-driven paradigm, while there are plenty of developers using low-resource PLs. On the other hand, there are few studies exploring the effects of multi-programming-lingual (MultiPL) pre-training for the code completion, especially the impact on low-resource programming languages. To this end, we propose the MultiCoder to enhance the low-resource code completion via MultiPL pre-training and MultiPL Mixture-of-Experts (MoE) layers. We further propose a novel PL-level MoE routing strategy (PL-MoE) for improving the code completion on all PLs. Experimental results on CodeXGLUE and MultiCC demonstrate that 1) the proposed MultiCoder significantly outperforms the MonoPL baselines on low-resource programming languages, and 2) the PL-MoE module further boosts the performance on six programming languages. In addition, we analyze the effects of the proposed method in details and explore the effectiveness of our method in a variety of scenarios.

==> contents/section2.tex <==
\section{Background and Motivation}
\label{sec:background}

\subsection{Pre-training for Programming Languages}
Inspired by the remarkable success of pre-training models in the field of NLP, many researchers trend to study the adaptation of pre-trained models to programming languages. One of the earliest attempts is CodeBert~\cite{feng2020codebert}, which is built on BERT~\cite{devlin2019bert} and pre-trained with six common programming languages (including Python, Java, JavaScript, PHP, Ruby, and Go). After that, PLBART~\cite{ahmad2021unified} follows the encoder-decoder architecture and learns multilingual representations of programming and natural language jointly. More recently, GraphCodeBert~\cite{guo2021graphcodebert} introduces two structure-aware pre-training tasks to model the structural information of source code. SYNCOBERT~\cite{wang2021syncobert} utilizes the contrastive learning~\cite{contrastive_learning} with two syntax-guided pre-training tasks to learn better code representation.

% With the rapid development of pre-trained models in programming languages, the progress of code intelligence has been greatly promoted. Some industrial products have already been implemented based on pre-training models, such as Copilot,\footnote{\url{https://copilot.github.com/}} an AI pair programmer which supports features such as code auto completion, converting comments to code, and auto-filling for repetitive code. The launch of these code intelligence products shows that the pre-training paradigm of programming languages is very promising. 

Unfortunately, most of the previous work has focused on mono-programming-lingual pre-training, which performs poorly on the tasks of low-resource programming languages. As mentioned in Section I, insufficient pre-training data for low-resource programming languages limits the performance on these languages. An effective way to improve the performance of low-resource programming languages is multi-lingual pre-training~\cite{devlin2019bert}.

\subsection{Multilingual versus Monolingual LMs}
With the success of monolingual English BERT models, the release of multilingual BERT~\cite{devlin2019bert} has led to widespread use of Transformer-based pre-trained multilingual LMs. Guo \textit{ea al.}~\cite{guo2019multilingualparaphrasing} introduces multilingual pre-training into decoder-only models. 
These studies demonstrate that multilingual pre-training models can effectively improve the performance of low-resource languages. 
However, multilingual LMs are still faced with some fundamental limitations~\cite{arivazhagan2019massively}.
% of multilingual LMs are pointed by recent works. 
Conneau \textit{et al.}~\cite{conneau2020unsupervised} find that adding more languages to a fixed model capacity will result in performance drops. This phenomenon is also called the curse of multilinguality (i.e., the lack of ability to represent all languages in a fair way), which can be alleaviated by increasing the model capacity~\cite{chau2020parsing}. Furthermore, Wu \textit{et al.}~\cite{wu2020all} also observe that the monolingual ability of a multilingual model decreases with smaller sizes of pre-training data. These limitations might result in the multilingual models underperforming the monolingual models when applied to a specific language~\cite{virtanen2019multilingual}. 
% For programming language pre-training models, Svyatkovskiy \textit{et al.}~\cite{svyatkovskiy2020intellicode} conduct several experiments on MultiPL models and MonoPL models, and the experimental results show that MultiPL models outperform MonoPL models on low-resource programming languages, while MonoPL models perform better on high-resource programming languages. 

%Although multilingual models can significantly improve the performance on low-resource languages or cross-lingual tasks, their performance loss on other languages is also non-negligible~\cite{johnson2017google,tan2018multilingual}.
Despite recent efforts have been taken to mitigate the limitations, the multilingual LMs are still struggling with how to balance the parameters across different languages~\cite{rust2021good}. To address the problem, we introduce Mixture-of-Experts modules to scale up the model capacity of the MultiPL pre-training.

\subsection{Mixture-of-Experts for Scaling Transformers}
The Transformer model~\cite{vaswani2017attention} is widely used in the NLP field,
% natural language processing, 
since it has proven obvious advantages over
% significantly outperforms 
other architectures such as Recurrent Neural Networks (RNNs). A Transformer layer consists of a Multi-Head Self-Attention module and a Feed-forward Network (FFN). Multiple Transformer layers are stacked one by one to constitute a Transformer model. More details about the Transformer model can be referred to~\cite{vaswani2017attention}. The computation of Transformer will increase proportionally with the increase of model parameters. An efficient method to scale up the Transformer is Mixture-of-Experts (MoE)~\cite{lepikhin2020gshard}. A typical MoE framework consists of a gated network and multiple expert sub-networks.
% \yp{, as shown in the upper right of Figure~\ref{fig:PL-MoE}}. 
The gated network calculates the proportion of the output of each expert network for an input $x$, and then adopts a weighted summation method to obtain the final output. The MoE can selectively activate a part of the parameters in the model for different inputs to participate in the calculation, so that the model can be scaled up to billions of parameters without a proportional increase in computation.

\subsection{Motivation for the Programming Language Specific Experts (PL-MoE)}
Although the MoE layer expands the model capacity, it does not take into account the exclusive features of different programming languages. In details, all the programming languages share the identical experts on each MoE layer. 
No matter the naive MoE~\cite{lepikhin2020gshard} or the Switch MoE~\cite{fedus2022switch}, the routing strategy of them is trained for token distribution rather than for different programming languages. Therefore, the MoE layers should be improved to guarantee the exclusive features of different programming languages. To protect the exclusive features of different programming languages, we propose a novel PL-level MoE routing strategy (PL-MoE) that provides PL-specific expert parameters. Meanwhile, a set of PL-shared experts are kept so that PL-agnostic knowledge can be learned, e.g. common literals used in various PLs.
% \yp{A visual comparison between the Switch MoE and the proposed PL-MoE is depicted in Figure~\ref{fig:PL-MoE}.}
% The motivation of introducing shared experts is to allow low-resource programming languages to still benefit from transferring knowledge at the MoE layer.

% Lepikhin \textit{et al.} propose Mixture-of-Experts Transformer model, which replaces the dense FFN layer with the MoE FFN layer. More details about MoE transformer are given in~\cite{lepikhin2020gshard}.
% The MoE layer consists of a gating network $\mathcal{G}_{i, E}$ and $E$ FFNs (i.e. expert), such that $\mathrm{FFN}_{1} \ldots \mathrm{FFN}_{E}$. 
% \begin{equation}
%     \mathcal{G}_{i, E}=\operatorname{GATE}\left(x_{i}\right)
%     \label{eqa:1}
% \end{equation}
% \begin{equation}
%     \mathrm{FFN}_{e}\left(x_{i}\right)=w o_{e} \cdot \operatorname{ReLU}\left(w i_{e} \cdot x_{i}\right)
%     \label{eqa:2}
% \end{equation}
% \begin{equation}
%     y_{i}=\sum_{e=1}^{E} \mathcal{G}_{i, e} \cdot \mathrm{FFN}_{e}\left(x_{i}\right)
%     \label{eqa:3}
% \end{equation}
% where $x_{i}$ is the input token at position $i$ to the MoE layer. The vector $\mathcal{G}_{i, E}$ is computed by the gating network. And it has one non-negative value for each expert, which determines the assignment of experts. And the ${FFN}_{e}$ (an expert) refers to a 2-layer fully-connected network using ReLU activation function, $w i_{e}$ and $w o_{e}$ refer to the input and output projection matrices for the $e$-th expert. 
